Cold nuclear matter effects on azimuthal decorrelation in heavy-ion collisions

The assumption of factorization lies at the core of calculations of medium effects on observables computable in perturbative Quantum Chromodynamics. In this work we examine this assumption, for which we propose a setup to study hard processes and bulk nuclear matter in heavy-ion collisions on the same footing using the Glauber modelling of heavy nuclei. To exemplify this approach, we calculate the leading-order corrections to azimuthal decorrelation in Drell-Yan and boson-jet processes due to cold nuclear matter effects, not considering radiation. At leading order in both the hard momentum scale and the nuclear size, the impact-parameter dependent cross section is found to factorize for both processes. The factorization formula involves a convolution of the hard cross section with the medium-modified parton distributions, and, for boson-jet production, the medium-modified jet function.

==> VJ/beamjet.tex <==
% Since we are dealing  with a typical SCET$_{II}$ problem, we need to introduce an additional regulator for rapidity (lightcone) singularities in beam and jet functions (as well as in the soft function). We adopt the $\eta$-regulator~\cite{Chiu:2011qc,Chiu:2012ir} in which 
% \begin{align}
% &\bar{n}_i\cdot\hat{P}\to \bar{n}_i\cdot\hat{P}\left(\frac{|\bar{n}_i\cdot\hat{P}|}{\nu}\right)^\eta\qquad\text{in the $n$-collinear Wilson line}\notag\\
% &n\cdot\hat{P}\to n\cdot\hat{P}\left(\frac{|2\hat{P}^3|}{\nu}\right)^\frac{\eta}{2}\qquad\text{in the soft Wilson line along $n$}.
% \end{align}
% Such a replacement leads to rapidity divergences of $1/\eta$ and a corresponding evolution in the rapidity renormalization scale $\nu$ that sums (large) rapidity logarithms. 

\section{Beam functions}

Employing the color neutrality of the initial hadronic states gives
\begin{align}\label{eq:beam_q}
 \langle P|(\phi_{n}^\dagger)^{\alpha'}_{a'}(x+t' \bar n)(\phi_{n})^{\alpha}_{a}(t \bar n)|P\rangle=  \frac{\delta_{a' a}}{d_C}\langle P|(\phi_{n}^\dagger)^{\alpha'}_{b}(x+t' \bar n)(\phi_{n})^{\alpha}_{b}(t \bar n)|P\rangle,
\end{align}
where $\phi_{n}$ stands for the collinear quark, antiquark or gluon fields, $\alpha$ and $\alpha'$ are the Lorentz or spinor indices and $a$ and $a'$ are the color indices for the fields in a $d_C$-dimensional representation of color $SU(N_c)$. The beam functions are given by projections of this quantity:
\begin{align}\label{eq:beam}
  &
  \langle P|(\phi_{n}^{f\dagger})^{\alpha'}_{a'}(x+t' \bar n)(\phi^f_{n})^{\alpha}_{a}(t \bar n)|P\rangle \notag\\
  &\hspace{2cm}=\frac{\delta_{a' a}}{d_C}\int_0^{1} \frac{d\xi}{\xi}~ \sum\limits_j{P}_{n, j}^{\alpha\alpha'} \mathcal{B}^j_{f/n}(\xi,b_T,\epsilon)e^{i \xi \bar n \cdot P\left( \frac{n\cdot x}{2}+t'-t \right)},
\end{align}
where the projectors ${P}_{n, j}^{\alpha \alpha'}$ for the parton flavor $f$ are given below. Using the momentum operator $\hat{P}$, one can write
\begin{align}\label{eq:beamcomp}
  \sum\limits_j{P}_{n, j}^{\alpha \alpha'} \mathcal{B}^j_{f/n}(\xi,b_T,\epsilon)&=
  2\xi \bar{n}\cdot P\langle P|(\phi_{n}^{f\dagger})^{\alpha'}_{a}(\vec{b}_T)\delta(\bar{n}\cdot \hat{P}-(1-\xi)\bar{n}\cdot P)(\phi^f_{n})^{\alpha}_{a}(0)|P\rangle\notag\\
  &\equiv 2\xi \bar{n}\cdot P\int\frac{dt}{2\pi}e^{-i\xi t\bar{n}\cdot P}\langle P|(\phi_{n}^{f\dagger})^{\alpha'}_{a}(t\bar{n} + b_T)(\phi^f_{n})^{\alpha}_{a}(0)|P\rangle\notag.
\end{align}

There are two independent gluon beam functions for unpolarized collisions. Let us define
\begin{align}
\mathcal{B}^{\alpha'\alpha}(\vec{b}_T)\equiv 2\xi \bar{n}\cdot P\int\frac{dt}{2\pi}e^{-i\xi t\bar{n}\cdot P}\langle P|\mathcal{B}^{a \alpha'}_{n \perp}(t\bar{n}+b_T)\mathcal{B}^{a \alpha}_{n \perp}(0) |P \rangle,
\end{align}
where the gluon field
\begin{align}
    \mathcal{B}^{a \alpha}_{n}=\frac{1}{g}W_{n}^\dagger i D_{n}^\mu W_{n}=\frac{1}{g}\biggl[\frac{1}{\bar{n}\cdot \mathcal{P}}W_n^\dagger[i\bar{n}\cdot D_n,i D_{n}^\mu]W_n\biggr]
\end{align}
with $\mathcal{P}$ the label momentum operator, $W_n$ the $n$-colinear Wilson line and $i D_{n}^\mu=i\partial^\mu+gA_n^\mu$.
% The two projectors ${P}_{n, j}^{\alpha' \alpha}$ with $j=1,2$ for gluon beam functions are completely determined by the symmetries of $\mathcal{B}^{\alpha'\alpha}(\vec{b}_T)$.
% Since the collinear gluons are transverse, there are at most 4 independent projectors at given $\vec{b}_T$. One of them has to be dependent of the others since  $\mathcal{B}^{\alpha'\alpha}$ is symmetric in its Lorentz indices. This can be easily seen by taking the complex conjugation of $\mathcal{B}^{\alpha'\alpha}$
% \begin{align}\label{eq:Bdagger}
%     \mathcal{B}^{\alpha'\alpha}(\vec{b}_T) &= (\mathcal{B}^{\alpha'\alpha})^*(\vec{b}_T)\notag=\langle P|\mathcal{B}^{a \alpha}_{n \perp}(0) \mathcal{B}^{a \alpha'}_{n \perp}(\vec{b}_T)|P \rangle=\langle P|\mathcal{B}^{a \alpha}_{n \perp}(-\vec{b}_T) \mathcal{B}^{a \alpha'}_{n \perp}(0)|P \rangle
% \end{align}
% and using the fact that
It respects rotational symmetries in the transverse plane and satisfies
\begin{align}\label{eq:rotation}
    \mathcal{B}^{\alpha'\alpha}(\vec{b}_T)={\Lambda(\theta)^{\alpha'}}_{\beta'}{\Lambda(\theta)^{\alpha}}_{\beta'}\mathcal{B}^{\beta'\beta}(\Lambda^{-1}(\theta)\cdot\vec{b}_T),
\end{align}
where the matrix $\Lambda(\theta)$ corresponds to the rotation by an angle $\theta$ around the $z$ axis. %According to the above two equations, rotating the system by $\theta=\pi$ gives
% \begin{align}
%     \mathcal{B}^{\alpha'\alpha}(\vec{b}_T)=\mathcal{B}^{\alpha\alpha'}(\vec{b}_T).
% \end{align}
Since the beam functions by definition are scalar functions, which are invariant under the rotation $\Lambda(\theta)$, the projectors should also respect the rotation symmetry in Eq. (\ref{eq:rotation}). This leaves us with two independent symmetric tensors: $g_T^{\alpha' \alpha}$ and $\frac{b_T^{\alpha'} b_T^{\alpha}}{b_T^2}$. Following \cite{Catani:2010pd, Becher:2012yn}, the two independent projectors are chosen to be:
\begin{align}
    {P}_{n, 1}^{\alpha \alpha'}= -\frac{1}{d-2}g_T^{\alpha' \alpha},\qquad {P}_{n, 2}^{\alpha \alpha'}=\frac{g_T^{\alpha\alpha'}}{d-2}-\frac{b_T^{\alpha} b_T^{\alpha'}}{b_T^2}.
\end{align}
From Eq. (\ref{eq:beamcomp}), one has
\begin{align}
    \mathcal{B}_{1,g} = -g_{T}^{\alpha\alpha'} \mathcal{B}_{\alpha'\alpha},\qquad \mathcal{B}_{2,g} = \biggl(\frac{d-2}{d-3}\biggr){P}_{n, 2}^{\alpha \alpha'}\mathcal{B}_{\alpha'\alpha}.
\end{align}

For collinear quarks or antiquarks, their beam functions are defined as the coefficients of
\begin{align}
P_{n}^{\alpha \alpha'}=
\frac{1}{2}\left(\slashed{n}\right)^{\alpha\alpha'} \xi \bar n \cdot P
\end{align}
From Eq. (\ref{eq:beamcomp}), one has
\begin{align}
\mathcal{B}_{f/n}(\xi, x_T^2,\epsilon)&=\int\frac{dt}{2\pi}e^{-i\xi t\bar{n}\cdot P}
\left<P\right|\bar\chi^f_{n}(t\bar n+x_T)\frac{\slashed{\bar{n}}}{2}\chi^f_{n}(0)\left|P\right>,\notag\\
\mathcal{B}_{\bar{f}/n}(\xi, x_T^2,\epsilon)&=-\int\frac{dt}{2\pi}e^{-i\xi t\bar{n}\cdot P}
\left<P\right|\bar\chi^f_{n}(0)\frac{\slashed{\bar{n}}}{2}\chi^f_{n}(t\bar n+x_T)\left|P\right>.
%\left<n\right|&\bar\chi^f_{n}(t'\bar n)\frac{\slashed{\bar{n}}_i}{2}\chi^f_{n}(x+t\bar n)\left|P\right>=\bar n\cdot P \int_{-1}^{0} d\xi \mathcal{B}_{f/N_1}(\xi, x_T^2,\mu) e^{-i \xi P\cdot( x+t \bar n-t'\bar{n}_i )}\nonumber\\
%&=-\bar n\cdot P \int_{0}^{1} d\xi \mathcal{B}_{\bar f/n}(\xi, x_T^2, \mu) e^{i \xi P\cdot( x+t \bar n-t'\bar{n}_i )}.
\end{align}
% $\frac{1}{2}\left(\slashed{n}_i\right)^{\alpha'\alpha}$ is the only Dirac matrix that gives the dominant (leading twist) contribution. Unlike the gluon case, $x_T^\mu$ seems hard to be used for the projection of the spinor representation of the Poincare group. One possible way to introduce the $x_T$ dependence is to choose a two-component spinor pointing along $\vec{x}_T$
% \begin{align}
%     \xi^\uparrow_x =\left( \begin{array}{c}
%          \cos\frac{\phi_x}{2}\\
%          \sin\frac{\phi_x}{2}
%     \end{array}\right)
% \end{align}
% and construct the four-component spinor, denoted by $u^\uparrow_x$ accordingly. The projector corresponding to (\ref{eq:proj2}) is
% \begin{align}
%     \frac{1}{2}\left(\slashed{n}_i\right)^{\alpha'\alpha} \xi \bar n \cdot P - 2 u^\uparrow_x \bar{u}^\uparrow_x = u^\downarrow_x \bar{u}^\downarrow_x - u^\uparrow_x \bar{u}^\uparrow_x.
% \end{align}

\section{Jet functions}


Now, let us definite the jet function in some jet algorithm using the WTA axis. In order to keep our discussion as general as possible, we only require the jet algorithm to respect factorization in SCET.  As discussed in Sec. \ref{sec:Zjet}, we choose a recoil-free jet axis to suppress non-global effects and constrict ourselves to azimuthal decorrelation in this subsection. In this case, we only need to include the jet collinear modes in the definition of our jet functions.

Given $m$ collinear consituents with momenta $\{p_{i}\}$, we would like to define a jet of transverse momentum $\vec{p}_{T,J}$ and rapidity $\eta_J$. Let us denote the operation of the jet algorithm on $\{p_{i}\}$ by two operators: $\vec{\hat{p}}_{T,J}$ and $\hat{\eta}_J$, which respectively give us the jet transverse momentum and rapidity. The jet function
 is defined as a function of $\vec{p}_{T,J}$ and $\eta_J$:
 \begin{align}\label{eq:jetdef_crude}
    &\frac{\delta_{a' a}}{2(2\pi)^{d-1}} \sum\limits_i P_{i}^{\alpha' \alpha} \mathcal{J}^i(\vec{b}_T, \vec{p}_{T,J}, \eta_J,\epsilon)\notag\\
    &
    =\left\langle 0\left|(\phi_{n})^{\alpha'}_{a'}\left(0\right)e^{i (\vec{\mathcal{P}}_T-\vec{p}_{J,T})\cdot \vec{b}_T}\delta^{(2)}\left(\vec{p}_{T,J}-\vec{\hat{p}}_{T,J}\right)\delta(\eta_J-\hat{\eta}_J)(\phi_{n}^\dagger)^{\alpha}_{a}\left(0\right)\right|0\right\rangle
\end{align}
with
\begin{align}\label{eq:Pjet}
P^{\alpha' \alpha}=\left\{
\begin{array}{ll}
-g_\perp^{\alpha'\alpha},\qquad g_\perp^{\alpha'\alpha}-2\frac{b_\perp^{\alpha'} b_\perp^{\alpha}}{b_\perp^2} &\text{for gluons},\\
\frac{1}{2}\left(\slashed{n}_J\right)^{\alpha'\alpha} \bar n \cdot p_J&\text{for quarks and antiquarks}.
\end{array}
\right. 
\end{align}
 Note that for the WTA is different from the collinear direction $n^\mu$, which, by definition, is aligned with the total momentum of the jet constituents $p_c^\mu$. In terms of its transverse momentum $\vec{p}_{T,c}$ and rapidity $\eta_c$, one has 
\begin{align}\label{eq:pc}
p^\mu_c=\left(\sqrt{p_{T,c}^2+p_c^2}\cosh \eta_c,\vec{p}_{T,c},\sqrt{p_{T,c}^2+p_c^2}\sinh \eta_c\right).
\end{align}
Here, we only focus on the back-to-back limit in which the difference between the WTA and SJA is small. Below, we multipole-expand the expression for the jet function in terms of such a small difference, as discussed in Sec. \ref{sec:Zjet}. 

% Then, the jet function is given by the decomposition of
% \begin{align}
%     &\left\langle 0 \left|(\phi_{n})^{\alpha'}_{a'}\left(\vec{b}_T\right)\delta^{(2)}\left(\vec{p}_{T,J}-\vec{\hat{p}}_{T,J}\right)\delta(\eta_J-\hat{\eta}_J)(\phi_{n}^\dagger)^{\alpha}_{a}\left(0\right)\right|0\right\rangle\notag\\
%     &\left\langle 0\left|(\phi_{n})^{\alpha'}_{a'}\left(0\right)e^{i \vec{\hat{p}}_T\cdot \vec{b}_T}\delta^{(2)}\left(\vec{p}_{T,J}-\vec{\hat{p}}_{T,J}\right)\delta(\eta_J-\hat{\eta}_J)(\phi_{n}^\dagger)^{\alpha}_{a}\left(0\right)\right|0\right\rangle.
% \end{align}
% Here we need to take out a phase factor $e^{i\vec{p}_{T,J}\cdot \vec{b}_T}$, which is combined with that of the vector boson transverse momentum into $e^{i\vec{q}_{T}\cdot \vec{b}_T}$.
%Here, we sum over the $n$-collinear states with a total four-momentum $p_c^\mu$.

In order to expand the right-hand side of Eq. (\ref{eq:jetdef_crude}) to linear order in $\phi_c$, we use the completeness relation for collinear states and write
\begin{align}
    &\frac{\delta_{a' a}}{2(2\pi)^{d-1}} \sum\limits_i P_{i}^{\alpha' \alpha} \mathcal{J}^i(\vec{b}_T, \vec{p}_{T,J}, \eta_J,\epsilon)=\sum\limits_{m=1}^\infty\prod\limits_{i=1}^m\left[\int\frac{d^d p_{i}}{(2\pi)^{d-1}}\delta^+(p_{i}^2)\right]  \notag\\
&\times J~\delta\left(\bar{n}\cdot p_c-\sum \bar{n}\cdot p_{i}\right)\delta^{(d-2)}\left(\sum \vec{p}_{i, \perp}\right)\Theta_{\text{in}}(\{p_{i}\})
  \notag\\
  &\times e^{i (\vec{p}_{c,T}-\vec{p}_{J,T})\cdot \vec{b}_T}\left\langle 0 \left|(\phi_{n})^{\alpha'}_{a'}\left(0\right)\right|\{p_{i},a\}\right\rangle \left\langle  \{p_{i},a\}\left|(\phi_{n}^\dagger)^{\alpha}_{a}\left(0\right)\right|0\right\rangle\end{align}
where $\Theta_{\text{in}}$ sets the in-cone condition for all the $n$-collinear partons in a corresponding jet algorithm,  $\delta^+(p^2)\equiv\delta(p^2)\theta(p^0)$, the total (collinear) momentum $p_c^\mu$ is given in Eq. (\ref{eq:pc})
and the Jacobian is defined as
\begin{align}
    J&\equiv \int_0^\infty dp_c^2d\eta_c d^2p_{c, T}\delta\left(n\cdot p_c-\sum n\cdot p_{i}\right)\delta^{(2)}\left(\vec{p}_{T,J}-\vec{\hat{p}}_{T,J}\right)\delta(\eta_J-\hat{\eta}_J).
\end{align}
Integrating out $p_c^2$ yields  
\begin{align}
    J= \int d\eta_c d^2p_{c, T} \bar{n}\cdot p_c\delta^{(2)}\left(\vec{p}_{T,J}-\vec{\hat{p}}_{T,J}\right)\delta(\eta_J-\hat{\eta}_J)
\end{align}
with $O(\delta\phi^2)$ terms neglected.


Let us carry out multiple expansion in $\delta\phi$ in order to further simplify $J$. We shall neglect all terms of $O(\delta\phi)$. In this case, the total $n$-collinear momentum aligns with
\begin{align}
    n^\mu = \left(1, \text{sech}~\eta_c\cos\phi_c,\text{sech}~\eta_c\sin\phi_c, \tanh\eta_c\right).
\end{align}
we choose the following two vectors to form a complete basis for the transverse ($\perp$) plane with respect to $n$
\begin{align}
&n^\mu_{\perp_1}=(0, \sin\phi_c, -\cos\phi_c, 0), &n^\mu_{\perp_2}=\left(0, \tanh\eta_c\cos\phi_c, \tanh\eta_c\sin\phi_c, -\text{sech}~\eta_c \right)
\end{align}
with
\begin{align}
    g_\perp^{\mu\nu} = -n_{\perp_1}^\mu n_{\perp_1}^\nu - n_{\perp_2}^\mu n_{\perp_2}^\nu.
\end{align}
Suppose that there are $m$ collinear partons in the jet respectively with momentum
%Let us consider the case with two collinear partons respectively with momenta
\begin{align}
P^\mu = \frac{\bar{n}\cdot p_c}{2} z_i n^\mu + p_{i, 1} n_{\perp_1}^\mu + p_{i, 2} n_{\perp_2}^\mu.
    % p_1^\mu = \frac{\bar{n}\cdot p_c}{2} z n^\mu + p_{1, 1} n_{\perp_1}^\mu + p_{1, 2} n_{\perp_2}^\mu, \qquad p_1^\mu = \frac{\bar{c}_\cdot p_c}{2} (1-z) n^\mu - p_{1, 1} n_{\perp_1}^\mu - p_{1, 2} n_{\perp_2}^\mu
\end{align}
In this choice of coordinates, our integration variables are $\{z_i, p_{i,1}, p_{i,2}\}$, $\eta_c$ and $\vec{p}_{c,T}$. We would like first to integrate out $\eta_c$ and $\vec{p}_{c,T}$. Here, since we only focus on azimuthal angle correlation, both $p_{i,1}$ and  $p{i,2}$ are assumed to scales as $\delta\phi$. If parton $1$ is the most energetic, one has, for the WTA merging scheme,
\begin{align}
    \eta_J = \eta_1, \qquad \vec{p}_{J, T} = (\sum\limits_i|\vec{p}_{i, T}|) \vec{n}_{1, T}.
\end{align}
Up to $O(\delta\phi)$, one can show that
\begin{align}
    &\hat\eta_J = \eta_c - \frac{p_{1,2}}{z_1 p_{c,T}},\notag\\
    &\vec{\hat{p}}_{J, T} = \vec{p}_{c, T} + \frac{p_{1,1}}{z_1 p_{c, T}}\left(p_c^y, -p_c^x\right)
\end{align}
and the Jacobian
\begin{align}
    \left|\frac{D\left(\hat{p}_{J}^x,\hat{p}_{J}^y,\hat{\eta}_J\right)}{D\left(\hat{p}_{c}^x,\hat{p}_{c}^y,\hat{\eta}_c\right)}\right|=1
\end{align}
where we have used $\sum\limits_i z_i=1$ and $\sum\limits_i p_{i,2}=0$ and 
\begin{align}
    |\vec{p}_{i, T}| = p_{i, 2} \tanh\eta_c+ z_i p_{c, T}.
\end{align}
From this, we have
\begin{align}
     J= \bar{n}_J\cdot p_J + 2 \frac{p_{1,2}}{z_1} \sinh\eta_J,
\end{align}
and
\begin{align}
    \vec{p}_{c,T}-\vec{p}_{J,T} = \frac{p_{1,1}}{z_1 p_{c, T}}\left(-p_c^y, p_c^x\right).
\end{align}
Since the remaining part of the integrand is obviously invariant under $p_{1,2}\to -p_{1,2}$, one can expect that such the $O(\delta\phi)$ term in $J$ can be dropped.

In jet algorithms with recoil free jet axis, for $\delta\phi\ll R$ the inclusion of $\Theta_{\text{in}}$ only gives rise to $R$-dependent sub-leading terms in $\delta\phi$. By further ignoring $\Theta_{\text{in}}$ we obtain the definition of the jet functions at leading order in $\delta\phi$
\begin{align}
    &\frac{\delta_{a' a}}{2(2\pi)^{d-1}} \sum\limits_i P_{i}^{\alpha' \alpha} \mathcal{J}^i(\vec{b}_T, \vec{p}_{T,J}, \eta_J,\epsilon)=\sum\limits_{m=1}^\infty\prod\limits_{i=1}^m\left[\int\frac{d^d p_{i}}{(2\pi)^{d-1}}\delta^+(p_{i}^2)\right]  \notag\\
&\times \bar{n}_J\cdot p_{J}~\delta\biggl(\bar{n}_J\cdot p_J-\sum \bar{n}_J\cdot p_{i}\biggr)\delta^{(d-2)}\left(\sum\vec{p}_{J_i, \perp}\right)
  \notag\\
  &\times e^{i (\vec{p}_{c,T}-\vec{p}_{J,T})\cdot \vec{b}_T}\left\langle 0 \left|(\phi_{n})^{\alpha'}_{a'}\left(0\right)\right|\{p_{i},a\}\right\rangle \left\langle  \{p_{i},a\}\left|(\phi_{n}^\dagger)^{\alpha}_{a}\left(0\right)\right|0\right\rangle\end{align}
  where we have replaced $\eta_c$ by $\eta_J$ and $p_c$ by $p_J$ everywhere else in the integrand on the right hand side except in the phase factor.

\section{Linear polarization and the hard function}

We can easily understand why the second term in the bracket does not contribute as long as there is only one collinear gluon Wilson line involved. Let us just take one (physical) polarization vector, say $\epsilon_1^\mu$, to be parallel to $b_T^\mu$, that is,
\begin{align}
\epsilon_1^{\mu} \epsilon_1^{\nu} =- \frac{b_T^{\mu} b_T^{\nu}}{b_T^2},
\end{align}
and choose the other polarization vector $\epsilon_2^\mu$ to be a vector orthogonal to $b_T, n_1, n_2$. Then, one has
\begin{align}\label{eq:proj2}
\left(g_T^{\mu\nu}-2\frac{b_T^{\mu} b_T^{\nu}}{b_T^2}\right) = \left(\epsilon_1^{\mu} \epsilon_1^{\nu} - \epsilon_2^{\mu} \epsilon_2^{\nu}\right).
\end{align}
If the observable does not have a preferential direction in the transverse plane, the second beam function shall not contribute.

To be more explicit, let us denote the on-shell amplitude for the $gq$ channel by $M^{\alpha\mu}$ with $\alpha$ and $\mu$ repectively the Lorentz indices of the photon and the gluon. Here, the color and the spin indices are suppressed, which shall be averaged (summed) over in the initial (final) states. For the on-shell massless photon, it can be shown that the two terms in the projector in front of the second beam function cancel with each other. If one repeats the same calculation for an off-shell photon, one has
\begin{align}
  g_{T\mu\mu'} g_{T\alpha\alpha'} M^{\alpha\mu} M^{*\alpha'\mu'} = -\frac{s^2+u^2 + 2 t m^2}{N s u}
\end{align}
with $p_\gamma^2 = m^2$
while
\begin{align}
\frac{{b_T}_{\mu} {b_T}_{\mu'}}{b_T^2}g_{T\alpha\alpha'} M^{\alpha\mu} M^{*\alpha'\mu'}=-\frac{s^2+u^2 - \frac{4 m^2 s\left(k_2 \cdot b_T\right)^2}{u b_T^2}}{2 N u s}.
\end{align}
Therefore, the projector $\left( \frac{g_{T\mu\mu'}}{2} - \frac{{b_T}_{\mu} {b_T}_{\mu'}}{b_T^2}\right)$ gives a non-zero result for a massive photon if $M^2$ is contracted with $g_{\alpha\alpha'}$. However, before we make any definite concolution, we have to make sure the above quality is the physical observable. That is, in the Drell-Yan process it is a lepton pair that is measured. We have to make sure that replacing this part of the diagrams by $g_{\alpha\alpha'}$ does not introduce any unphysical contribution. Let us calculate the whole process: $g(p_1), q(p_2)\to \gamma^*(k_1 = l_1 + l_2), J(k_2)$.

In $Z$-jet production, one has a similar result. After some algebra, one can show that for $gq\to Z^0 q$
\begin{align}
    &\epsilon_{T\mu}\epsilon_{T\mu'} M^{\alpha\mu} M^{*\alpha'\mu'}\left(\frac{p_{Z\alpha} p_{Z\alpha'}}{M_z^2}-g_{\alpha\alpha'}\right)\\
    &=-\frac{8 \pi ^2 \alpha_{EM}\alpha_S e_q^2}{n}\left[\frac{4 M_Z^2 (p_Z\cdot \epsilon_T)^2}{\hat{u}^2}+\frac{\hat{u}}{\hat{s}}+\frac{\hat{s}}{\hat{u}}
    \right]
\end{align}
after averaging (summing) over color and spin indices in the initial (final) states. Here, the physical (transverse) polarization represents $\epsilon_{1,2}$ above and
\begin{align}
e _ { q } ^ { 2 } \rightarrow \frac { \left( 1 - 2 \left| e _ { q } \right| \sin ^ { 2 } \theta _ { W } \right) ^ { 2 } + 4 e _ { q } ^ { 2 } \sin ^ { 4 } \theta _ { W } } { 8 \sin ^ { 2 } \theta _ { W } \cos ^ { 2 } \theta _ { W } }.
\end{align}
The transverse hard function, corresponding to the standard beam function, is given by the sum over the two physical polarizations, that is,
\begin{align}
    |\bar{M}_{gq\to Z^0 q}|^2 = -\frac{16 \pi ^2 \alpha_{EM}\alpha_S e_q^2}{n}\left[\frac{2 M_Z^2 p_T^2}{\hat{u}^2}+\frac{\hat{u}}{\hat{s}}+\frac{\hat{s}}{\hat{u}}
    \right]
\end{align}
with $p_T^2 = \hat{u}\hat{t}/\hat{s}$. According to (\ref{eq:proj2}), the hard function for the second beam function is given by
\begin{align}
    |\bar{M}_{gq\to Z^0 qL}|^2 &= -\frac{32 \pi ^2 \alpha_{EM}\alpha_S e_q^2}{N_c}M_Z^2 \frac{(p_Z\cdot \epsilon_1)^2 - (p_Z\cdot \epsilon_2)^2}{\hat{u}^2}.
\end{align}
In our choice of the coordinate, $\epsilon_1^\mu\propto b_T^\mu$ is orthogonal to $p_Z^\mu$ while $\epsilon_2$ is parallel to $b_T$. Hence,
\begin{align}
    |\bar{M}_{gq\to Z^0 qL}|^2 &= \frac{32 \pi ^2 \alpha_{EM}\alpha_S e_q^2}{N_c}M_Z^2 \frac{p_T^2}{\hat{u}^2}= \frac{32 \pi ^2 \alpha_{EM}\alpha_S e_q^2}{N_c}M_Z^2 \frac{\hat{t}}{\hat{u}\hat{s}}.
\end{align}
In general, we have
\begin{align}
    %\nonumber\\
     |\bar{M}_{gq\to Z^0 qL}|^2 &=-\frac{32 \pi ^2 \alpha_{EM}\alpha_S e_q^2}{N_c}M_Z^2 \frac{2(p_Z\cdot \epsilon_1)^2 - p_T^2}{\hat{u}^2}\nonumber\\
    &=\frac{32 \pi ^2 \alpha_{EM}\alpha_S e_q^2}{N_c}M_Z^2\left[\frac{\hat{t}}{\hat{u}\hat{s}} + 2 \frac{(p_Z\cdot b_T)^2}{\hat{u}^2 b_T^2}\right]
\end{align}
From this, we can see that if the observable has a rotational symmetry in the transverse plane, one can replace $b_T^\mu b_T^\nu$ by $\frac{1}{2} b_T^2 g_T^{\mu\nu}$ and has
\begin{align}
    |\bar{M}_{gq\to Z^0 qL}|^2 \to \frac{32 \pi ^2 \alpha_{EM}\alpha_S e_q^2}{N_c}M_Z^2\left[\frac{\hat{t}}{\hat{u}\hat{s}} - \frac{p_T^2}{\hat{u}^2}\right]=0.
\end{align}
Otherwise, the second beam function should contribute the observable, such as the azimuthal angle decorrelation. The result for $q\bar{q}\to Z^0 g$ is given by the crossing symmetry: $\hat{s}\to \hat{u}, \hat{t}\to \hat{s}, \hat{u} \to \hat{t}$, color factor $\frac{1}{N_c (N_c^2-1)} \to \frac{1}{N_c^2}$ and an overall minus sign for taking a quark from the final state to the initial state.

\subsubsection{From $\vec{b}_\perp$ to $\vec{b}_T$}
The above derivation of hard function is valid also for case with the projector in (\ref{eq:proj2}) replaced by the projector in (\ref{eq:Pjet}), which is orthogonal to $n_J$ and $\bar{n}_J$. Similarly, the linearly polarized gluon jet function is also defined in terms of this projector. Since we are only interested in transverse observables, we multipole-expand it in both hard and jet function to get $b_T$-dependence instead. Since the coordinates $b^\mu\sim (1,1, 1/\lambda)/Q$, one simply replaces all the $\vec{b}_\perp\equiv(b_1, b_2)$ by
\begin{align}
    &b_1= -n_{\perp_1}\cdot b \to -n_{\perp_1}\cdot b = b_x \sin\phi_J - b_y \cos\phi_J,\notag\\
    &b_2= -n_{\perp_2}\cdot b \to -n_{\perp_2}\cdot b = b_x \cos\phi_J\tanh\eta_J + b_y \sin\phi_J\tanh\eta_J.
\end{align}
Our choice of the coordinates corresponds to $\phi_J=\pi/2$, that is,
\begin{align}
    b_1 = b_x,\qquad b_2 = by \tanh\eta_J.
\end{align}
The longitudinal gluon jet function at one-loop takes the form
\begin{align}
    \mathcal{J}_{g,2}^{(1)}(b,\mu,\nu) & = \left(- \frac{1}{3}C_A + \frac{2}{3} T_F n_f\right) \frac{b_x^2 - b_y^2\tanh^2\eta_J}{b_x^2 + b_y^2\tanh^2\eta_J},
\end{align}
while other jet functions depend only on $b_x$.
Keeping $\vec{b}_T$-dependence in hard and linearly polarized jet functions one can study azimuthal asymmetric in $\vec{q}\equiv \vec{p}_{J,T}+\vec{p}_{V,T}$.
